The BigScience ROOTS Corpus: A 1.6TB Composite Multilingual Dataset

As language models grow ever larger, the need for large-scale high-quality text datasets has never been more pressing, especially in multilingual settings. The BigScience workshop, a 1-year international and multidisciplinary initiative, was formed with the goal of researching and training large language models as a values-driven undertaking, putting issues of ethics, harm, and governance in the foreground. This paper documents the data creation and curation efforts undertaken by BigScience to assemble the Responsible Open-science Open-collaboration Text Sources (ROOTS) corpus, a 1.6TB dataset spanning 59 languages that was used to train the 176-billion-parameter BigScience Large Open-science Open-access Multilingual (BLOOM) language model. We further release a large initial subset of the corpus and analyses thereof, and hope to empower large-scale monolingual and multilingual modeling projects with both the data and the processing tools, as well as stimulate research around this large multilingual corpus.

==> extras/checklist.tex <==
\newpage

\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section\ref{sec:ethics}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Complete listing in Appendix and Dataset Cards}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See Section\ref{sec:ethics}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Section~\ref{section:common_crawl_section}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Section~\ref{section:obtaining}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

\newpage

==> extras/corpus_linguistics.tex <==
\paragraph{Corpus Linguistics} 

The basic idea of transfer learning assumes that properties of one task/dataset could be re-used in another. In case of language models, their pre-training corpora are implicitly assumed to have the linguistic properties that are useful in the target task (although in practice the current language models struggle to acquire the phenomena that are the more rare in the training data \citep{ZhangWarstadtEtAl_2021_When_Do_You_Need_Billions_of_Words_of_Pretraining_Data}). This echoes the corpus linguistics tradition, with the major difference that a big part of that tradition was deciding what exactly should be represented, and how to best sample textual data to achieve such representation. In particular, the major national corpora such as the British \citep{Leech_1992_100_million_words_of_English_British_National_Corpus_BNC}, American \citep{MacleodIdeEtAl_2000_American_National_Corpus_Standardized_Resource_for_American_English}, Japanese \citep{Maekawa_2008_Balanced_Corpus_of_Contemporary_Written_Japanese} and other national corpora were painstakingly collected over the years to to serve as balanced samples of the different genres of spoken and written speech produced at a given point in time, negotiating exemptions with copyright holders. Corpus linguistics has contributed methodology and tools for statistical analysis of linguistic data (such as concordances on plain and annotated corpora \citep{Anthony_2013_Developing_AntConc_for_new_generation_of_corpus_linguists}, frequency-based analysis \citep{LeechRayson_2014_Word_frequencies_in_written_and_spoken_English_Based_on_British_National_Corpus,Kilgarriff_2001_Comparing_Corpora}, word sketches \citep{KilgarriffTugwell_2002_Sketching_words}, collocations \citep{BrezinaMcEneryEtAl_2015_Collocations_in_context_new_perspective_on_collocation_networks}, collostructions \citep{StefanowitschGries_2003_Collostructions_Investigating_interaction_of_words_and_constructions} etc.). Corpus linguistics methodology is widely used in language pedagogy \citep{Sinclair_2004_How_to_use_corpora_in_language_teaching}, lexicography \citep{Teubert_2007_Corpus_linguistics_and_lexicography}, sociolinguistic research \citep{ReppenFitzmauriceEtAl_2002_Using_corpora_to_explore_linguistic_variation} etc. Its contributions in creating representative samples of textual data and negotiating the copyright difficulties is also very relevant to the NLP dataset practice, and its research on statistical association measures \citep{Rychly_2008_LexicographerFriendly_Association_Score,Brezina_2018_Statistical_choices_in_corpus-based_discourse_analysis} is also key to the fundamental research on distributional semantics.


% \subsection{Frequency analysis.} One of the standard tools of classical corpus linguistic analysis is analysis of ngram frequencies. The tools developed in scope of this project currently support unigram, bigram and trigram frequency analysis. As an illustration, Fig X shows the top\footnote{Excluding stopwords, which came from NLTK and Spacy stopword lists for English, French, Spanish and Arabic, and from online sources for Bengali. See App. TODO for full details.} 50 unigrams for 5 languages (English, French, Spanish, Arabic and Bengali) together with their frequency per million tokens. Analysis of top frequent ngrams allows to see which concepts are more characteristic of a given subcorpus. In this case, we can see that e.g. Paris is one of the top ngrams in the French Wikipedia, but not the others. 

% Another type of analysis that this tool allows for is comparative analysis of a specific vocabulary set across languages. As a brief illustration, Table TODO shows the relative frequencies per million token for the days of the week in the Wikipedias for the same languages. This shows TODO.

==> extras/documentation_related_work.tex <==
Documentation of datasets used for training language models is an important but often overlooked part of the pipeline ranging from data gathering to model deployment. However, there have been relevant documentation efforts both within the ML community and in related communities such as corpus linguistics-- we provide a brief overview of them in the current section.

\paragraph{Documentation in the broader ML community.} The importance of documentation has become a central point of discussion, triggered by several complementary directions of research, ranging from studies on the usage of datasets and how poor documentation has led to multiple versions and subsets of datasets being used concurrently and sometimes interchangeably~\cite{koch2021, raji2021ai}. This was further supported by investigations of datasets such as ImageNet~\citep{deng2009imagenet} that were found to contain deeply problematic images and categories, including sexist and racist categories and images of poor quality, some with explicit nudity~\citep{prabhu2020large,crawford2019excavating}. Studies of multimodal datasets such as LAION-400M~\cite{Schuhmann2021} have found similar results, of images and text representing pornography, malign stereotypes, and racist slurs~\cite{Birhane2021}, underlining the importance of proper dataset analysis and documentation. Other datasets that have been documented and analyzed include the Common Crawl \citep{Dodge2021}, C4 \citep{luccioni2021s,Kreutzer2022} and BookCorpus \cite{bandy2021addressing}. While this kind of documentation is far from standard practice, it is becoming increasingly common given recent calls for better documentation~\citep{rogers-2021-changing, bender2021} as well as empirical studies on data memorization in language models (e.g.~\citet{carlini2019secret,carlini2022quantifying}).


\paragraph{Documentation practice proposals.} Many approaches have been proposed for providing documentation and information to accompany ML datasets. Initial work has proposed static datasheets for general ML datasets~\citep{gebru2021datasheets} and data statements for textual datasets in NLP specifically~\citep{bender2018data}. Complementary initiatives include work on Factsheets for both models and datasets ~\citep{arnold2019factsheets,hind2020experiences,richards2020methodology} as well as more complete documentation of all of the steps in the data creation and implementation cycle (as opposed to only the final product), which aims to improve accountability and transparency~\citep{hutchinson2021towards}. Finally, recent work on dataset deprecation has also proposed improved documentation of this process via deprecation sheets and a centralized repository for hosting them~\citep{luccioni2022}. All of this work underlines the increased attention towards better documentation of ML datasets during the entirety of their lifecycle, from creation to sunsetting.

%\paragraph{Dataset Governance.} The oversight and governance of datasets has also come to the forefront of research efforts, with notable efforts aiming to advocate for improved dataset stewardship~\citep{Peng2021} and data-driven language governance~\citep{jernite2022governance}. \textbf{TODO: Yacine, maybe you want to add something here?}

\paragraph{Documenting textual corpora in NLP.} An inspiration for our work is a recent emphasis on a more in-depth documentation of what is included in the corpora used for training NLP models in general, and large language models in particular. The most notable example of this is the Pile \citep{Gao2020}, a curated dataset for language modeling that has become widely used for training state-of-the-art English-language models \citep{lieber2021jurassic,Smith2022,black2022gpt,zhang2022opt}. In addition to releasing a datasheet \citep{Biderman2022}, the authors analyze and document a variety of syntactic and semantic properties of the dataset including structural statistics (n-gram counts, language, document sizes), topical distributions across its components, social bias and sentiment co-occurrence, pejorative content, and information about licensing and authorial consent. Following \citep{biderman2020pitfalls,prabhu2020large} and anticipating \citet{Birhane2021Values}, they identify empowering users of their data and models trained on their data to make informed decisions as their primary goal.


Above and beyond the efforts described above, data documentation has been a major part of disciplines such as data studies and science and technology studies (STS)~\cite{iliadis2016critical, hey2009fourth}. Elements of data documentation have also been increasingly adopted in conference submission checklists for conferences such NAACL 2021, NAACL 2022 Responsible NLP checklist~\cite{rogers-etal-2021-just-think}, and datasets have also been increasingly central to conferences such as NeurIPS.

==> section_5_RETIRED.tex <==
% \section{Postprocessing:  filtering, PII}



% \textcolor{red}{(This section will be removed and its contents moved to sections 3 and 4}

% Filtering / cleaning / dedup:
% \begin{itemize}
%     \item Need to apply a final set of filters, cleaning and dedup scripts on all collected datasets (pseudo\_crawl divided by website domain and data catalogue). Definitions:
% \begin{itemize}
% \item Filtering: Rule that determines whether or not an example should be kept in the dataset
% \item Cleaning: An operation that modifies an example to remove or correct unwanted patterns
% \item Deduplication: An operation that allows to keep only a single instance of a group of similar instances.
% \end{itemize}
%     \item why? We wish to have as textual data natural language by human for humans (except for identified code examples)
%     \item List of all the pre-processing functions used: \url{https://huggingface.slack.com/archives/C0307KE5UNT/p1648677158777079?thread_ts=1647958570.924839&cid=C0307KE5UNT} 
%     \item We have developed a pipeline that allows us to flexibly code methods to filter, clean or de-duplicate. We can then select which operations should be applied to which datasets and observe the modifications generated on a subset of the datasets as well as some estimated statistics (percentage of examples filtered out / deduplicated / modified). 
%     \item We determined the necessary post processing methods by manual observations of the dataset. The developed pipeline allowed us to manually check that there were no undesirable effects to the methods developed for a specific problem. 
% \end{itemize}
% Lucile, Thomas, Roman, Sasha and Meg
% Leandro, Chris, Hugo, Teven

==> tables/documents-removed.tex <==
\begin{tabular}{@{}cc@{}} 
  \small
 \toprule
 Lang.   & R. Docs. \\
 \midrule
 BN & 48.8 \% \\
 HI & 25.7 \% \\
 ZH & 23.1 \% \\
 VI & 21.3 \% \\
 CA & 21.1 \% \\
 AR & 20.3 \% \\
 EN & 17.2 \% \\
 FR & 17.0 \% \\
 ES & 16.9 \% \\
 UR & 15.8 \% \\
 PT & 12.6 \% \\
 ID & 10.4 \% \\
 EU & \phantom{0}5.2 \% \\
 \bottomrule
\end{tabular}
